Re-mapping the Internet: Bring the IXPs into Play

The Internet topology is of high importance in designing networks and architectures, evaluating performance, and economics. Interconnections between domains (ASes), routers, and points of presence (PoPs), have been measured, analyzed, and modeled. However, existing models have some serious shortcomings, related to ease, accuracy and completeness of measurements, and limited applicability to emerging research areas. To this end, in this paper, we propose a novel approach towards capturing the inter-domain Internet topology. Motivated by the recent interest in the Internet eXchange Points (IXPs), we introduce a network graph model based on IXPs and their AS memberships. The proposed model aims to complement previous modeling efforts, shed light on unexplored characteristics of the Internet topology, and support new research directions. We also collect and make available Internet connectivity data, analyze main topological properties, and discuss application-related issues.

==> Applications.tex <==
We now discuss how the proposed IXP-based models (Section~\ref{sec:model}) and the findings of our analysis (Section~\ref{sec:dataset-analysis}) can be applied to Internet research problems. In particular, we focus on three main research areas: (a) inter-domain routing, (b) IXP-related innovation, and (c) network economics. We present $X$ example cases (each of them belonging to one of the aforementioned areas), where we use our model and conclusions, to design better networks, optimize the performance ..., select policies ..., etc. As we show in this section, our model can be a important tool in both technical and economic oriented Internet studies.

\subsection{Inter-domain routing}
\blue{how can we use findings to provide insights about Performance evaluation, connectivity, design of protocols, outsourcing services, etc.? - Think of applications!}

\textbf{Extending the AS-graph.} The AS-graph is built from routes/paths advertised by the BGP protocol. Since in BGP messages (from which we retrieve the edges of the AS-graph) only \textit{one} -the ``best''- path appears, it follows that some connectivity information will be missing from the resulting AS-graph. For instance, even if an AS has a backup link with another AS (public -over an IXP- or private peering), the corresponding connection/edge will not be included in the graph. As a result, the constructed AS-graph could be considered as a \textit{lower bound} or an \textit{understimation} of the Internet's connectivity.

On the other hand, in an IXP-based graph, it might happen that two ASes are both connected to the same IXP, but they do not peer (or are connected, in general, cf. c2p policies) with each other. Hence, although one can traverse in the IXP-graph from one AS to another through a common IXP, it is not always true that this path exists in reality (due to policies or an absence of connectivity). Therefore, when considering a routing process, if we assume all the possible paths in the IXP-graph, we will tend to \textit{overestimate} the networking possibilities, e.g., path diversity.

Despite the limitations of both approaches, they can be combined towards a more complete evaluation of network protocols, services, etc. Using only the AS-graph could serve as a lower bound of performance, whereas using the aggregated AS- and IXP- graphs will be an upper bound for it. Hence, the performance will lie in the range between these bounds, in contrast to most approached that only lower bound it, by using only the AS-graph.

\blue{[TODO: Include some of our analysis findings to say sth useful and/or interesting about this problem.]}

\subsection{IXP-related innovation}
IXPs have been recently attracting a lot of attention, due to ..., e.g., []. As a result, a number of interesting problems and research directions appeared. Using an IXP multigraph, such problems can be tackled in an easier, more structured, and more complete manner.

\textbf{Clouds/Middleboxes at IXPs.} Outsourcing middleboxes to the cloud has been recently proposed as a novel way to decrease infrastructure, costs, management, etc., for enterprises~\cite{Sherry-Making-Middleboxes-CCR-2012}. Traffic of an enterprise is directed to a middlebox service located at a cloud facility and then redirected to its source or destination. Identical locations for installing such middleboxes are IXPs, because they (i) offer access to a number of ASes (and their customers) and, thus, to a large number of (potential) clients, (ii) ensure good connectivity (high bandwidth, availability, etc.), (iii) are independent of a single AS (i.e., providers of enterprises do not need to pay transit for this traffic), (iv) are usually colocated with a cloud facility(?).

An interesting question that the designer of the above system needs to answer is: ``At which IXP to place t middlebox service?''. A simple algorithm giving an initial answer to this problem could be the following:\\
(a) correspond: enterprise / potential client $\rightarrow$ AS (multiple enterprises, increase the weight of an AS)\\
(b) correspond: (weighted) AS $\rightarrow$ IXP\\
(c) chose IXP, based on its total weight, location, price, etc.

\blue{[TODO: show how our analysis, e.g., which metrics, can be used by this algorithm]}


\subsection{Network economics}


\textbf{A ``transit-free'' Internet (a.k.a. A p2p AS network).} Peeringy policies (cf. valley-free models) dictate that an AS can announce prefixes belonging to itself and its customers, but not prefixes of its peers. Therefore, an AS communicates with a non-peer or non-customer AS through a transit AS, which charges the traffic crossing it. However, as has been shown, peering policies in reality is much more complex than p2p or c2p, and the valley-free model is often violated. This indicates that peering ASes agree to allow traffic generated from / destined to IPs not belonging under their peers' networks. 

Adopting such policies greatly affects Internet routing and can have a great effect on the network economics as well. For instance, in Fig.~\ref{fig:transit-free} AS-2 can exchange traffic with AS-5 through their transit AS-1, and the same holds for traffic between AS-3 and AS-4. However, the peering AS-2 and AS-3 could agree to forward traffic from their peers (AS-4 and AS-5, respectively) to each other. Thus they could mutually benefit from this agreement and reduce the transit costs they pay to AS-1.

An AS in order to select with which AS it will peer, or to which IXP it will become member, can evaluate the potential benefits from such peerings/memberships. The IXP graph can be a useful tools towards this direction. E.g., ... . 

\underline{Extra:} Maybe remove the tier-1 ASes (or the ASes that exclusively offer transit to other ASes) to see how the Internet topology changes, or, in other words, how a ``transit-free'' Internet topology could be. Would there be enough connectivity or more things need to be done?

\begin{figure}
\includegraphics[width=\linewidth]{./figures/transit_free_example}
\caption{Transit-free example}
\label{fig:transit-free}
\end{figure}


\textbf{Selecting a new IXP connection.} Algorithm:\\
(a) correspond: ASes for (potential) peering (could be, e.g., traffic-related, e.g., ASes that are content providers) $\rightarrow$ IXPs\\
(b) chose IXP, based on its total weight, location, price, etc.


